Universal quantification makes automatic structures hard to decide

Automatic structures are first-order structures whose universe and relations can be represented as regular languages. It follows from the standard closure properties of regular languages that the first-order theory of an automatic structure is decidable. While existential quantifiers can be eliminated in linear time by application of a homomorphism, universal quantifiers are commonly eliminated via the identity $\forall{x}. \Phi \equiv \neg (\exists{x}. \neg \Phi)$. If $\Phi$ is represented in the standard way as an NFA, a priori this approach results in a doubly exponential blow-up. However, the recent literature has shown that there are classes of automatic structures for which universal quantifiers can be eliminated by different means without this blow-up by treating them as first-class citizens and not resorting to double complementation. While existing lower bounds for some classes of automatic structures show that a singly exponential blow-up is unavoidable when eliminating a universal quantifier, it is not known whether there may be better approaches that avoid the na\"ive doubly exponential blow-up, perhaps at least in restricted settings. In this paper, we answer this question negatively and show that there is a family of NFA representing automatic relations for which the minimal NFA recognising the language after eliminating a single universal quantifier is doubly exponential, and deciding whether this language is empty is EXPSPACE-complete. The techniques underlying our EXPSPACE lower bound further enable us to establish new lower bounds for some fragments of B\"uchi arithmetic with a fixed number of quantifier alternations.

==> config/ABACABA-word-utils.tex <==
\makeatletter
\def\SOUL@ulstunderline#1{{%
    \setbox\z@\hbox{#1}%
    \dimen@=\wd\z@
    \dimen@i=\SOUL@uloverlap
    \advance\dimen@2\dimen@i
    \rlap{% Draw underline
        \null
        \kern-\dimen@i
        \SOUL@ulcolor{\SOUL@ulleaders\hskip\dimen@}%
    }%
    %\SOUL@ulpreamble% Switch to draw over-strike
    \advance\SOUL@uldp2pt
    \advance\SOUL@ulht-2pt
    \rlap{%
        \null
        \kern-\dimen@i
        \SOUL@ulcolor{\leaders\hrule\@depth\SOUL@uldp\@height\SOUL@ulht\relax\hskip\dimen@}%
    }%
    \unhcopy\z@
}}
\def\SOUL@ulsteverysyllable{%
    \SOUL@ulstunderline{%
        \the\SOUL@syllable
        \SOUL@setkern\SOUL@charkern
    }%
}
\def\SOUL@ulstsetup{%
    \SOUL@ulsetup
    \let\SOUL@everysyllable\SOUL@ulsteverysyllable
}
\DeclareRobustCommand*\ulII{\SOUL@ulstsetup\SOUL@}

\makeatletter

%% Alphabet symbols
\NewDocumentCommand{\comb}{ m }{\mathObject{Comb}[#1][]{}}
\NewDocumentCommand{\combInner}{ m }{\mathObject{Comb}[#1][\prime]{}}

\NewDocumentCommand{\wLetterInner}{ m }{{\normalfont{\texttt{{#1}}}}}
\NewDocumentCommand{\wLetterInnerAux}{m}{{\normalfont{\texttt{\textbf{#1}}}}}
%\NewDocumentCommand{\wA}{}{\wLetterInner{\rotatebox[origin=c]{180}{A}}}
\NewDocumentCommand{\wA}{}{\wLetterInner{A}}
\NewDocumentCommand{\wEncodingPrefix}{}{\wA}
\NewDocumentCommand{\wRB}{}{\wLetterInnerAux{\kern0pt\textlbrackdbl\kern0pt}}
\NewDocumentCommand{\wRE}{}{\wLetterInnerAux{\kern0pt\textrbrackdbl\kern0pt}}
\NewDocumentCommand{\wCB}{}{\wLetterInnerAux{\kern-0.5pt\textlangle\kern0.5pt}}
\NewDocumentCommand{\wCE}{}{\wLetterInnerAux{\kern0.5pt\textrangle\kern-0.5pt}}
\NewDocumentCommand{\wSharp}{}{\wLetterInner{\#}}
\NewDocumentCommand{\wBlank}{}{\wLetterInner{\textvisiblespace}}
\NewDocumentCommand{\wDots}{}{{\color{lightgray}\cdots}}
\NewDocumentCommand{\wPref}{ s m }{{\IfBooleanTF{#1}{\color{cADarker}}{\color{cADark}}#2}}
\NewDocumentCommand{\wSuf}{ s m }{{\IfBooleanTF{#1}{\color{cDDarker}}{\color{cDDark}}#2}}
\NewDocumentCommand{\wRedC}{ m }{{\color{cA!85!black}#1}}
\NewDocumentCommand{\wBlueC}{ m }{{\color{cD!80!black}#1}}
\NewDocumentCommand{\wOut}{ m }{\text{\begingroup\setulcolor{black}\ul{\mbox{\ensuremath{#1}}}\endgroup}}
\NewDocumentCommand{\wOutD}{ m }{\text{\begingroup\setul{3.5pt}{1.0pt}\setulcolor{black}\ul{\mbox{\ensuremath{#1}}}\endgroup}}
\NewDocumentCommand{\wRed}{ m }{\text{\begingroup\setulcolor{cA}\ul{\mbox{\ensuremath{#1}}}\endgroup}}
\NewDocumentCommand{\wBlue}{ m }{\text{\begingroup\setulcolor{cD}\ul{\mbox{\ensuremath{#1}}}\endgroup}}
\NewDocumentCommand{\wRedII}{ m }{\text{\begingroup\setulcolor{cA}\ulII{\mbox{\ensuremath{#1}}}\endgroup}}
\NewDocumentCommand{\wBlueII}{ m }{\text{\begingroup\setulcolor{cD}\ulII{\mbox{\ensuremath{#1}}}\endgroup}}
\NewDocumentCommand{\wRedD}{ m }{\text{\begingroup\setul{3.5pt}{1.0pt}\setulcolor{cA}\ul{\mbox{\ensuremath{#1}}}\endgroup}}
\NewDocumentCommand{\wBlueD}{ m }{\text{\begingroup\setul{3.5pt}{1.0pt}\setulcolor{cD}\ul{\mbox{\ensuremath{#1}}}\endgroup}}
\NewDocumentCommand{\wRedDD}{ m }{\text{\begingroup\setul{3.5pt}{1.0pt}\setulcolor{cA}\ulII{\mbox{\ensuremath{#1}}}\endgroup}}
\NewDocumentCommand{\wBlueDD}{ m }{\text{\begingroup\setul{3.5pt}{1.0pt}\setulcolor{cD}\ulII{\mbox{\ensuremath{#1}}}\endgroup}}


\NewDocumentCommand{\w}{ m }{\wLetterInner{#1}}
%\NewDocumentCommand{\wTile}{ m }{\kern2pt{#1}\kern1pt}

\NewDocumentCommand{\wordLogN}{}{2}
\NewDocumentCommand{\wordN}{}{4}

\NewDocumentCommand{\wWordIV}{}{40102010301020104}

\NewDocumentCommand{\wExampleWordIV}{ m m }{\,\w{\StrMid{40102010301020104}{1}{#1}[\myResult]\setulcolor{cA}\ul{\myResult}}\setulcolor{cBLight}\,#2\,\w[cB]{\StrMid{40102010301020104}{#1+1}{17}[\myResult]\setulcolor{cD}\ul{\myResult}}\,\wA\wA\,}

% Gamma
\NewDocumentCommand{\wYin}{}{\w{x}}%{↓}
%\NewDocumentCommand{\wYin}{}{\w{\textuparrow}}%{↓}
\NewDocumentCommand{\wYang}{}{\w{y}}%{↑}
%\NewDocumentCommand{\wYang}{}{\w{\textdownarrow}}%{↑}
